Introducing Spectral Attention for Long-Range Dependency in Time Series Forecasting

Sequence modeling faces challenges in capturing long-range dependencies across diverse tasks. Recent linear and transformer-based forecasters have shown superior performance in time series forecasting. However, they are constrained by their inherent inability to effectively address long-range dependencies in time series data, primarily due to using fixed-size inputs for prediction. Furthermore, they typically sacrifice essential temporal correlation among consecutive training samples by shuffling them into mini-batches. To overcome these limitations, we introduce a fast and effective Spectral Attention mechanism, which preserves temporal correlations among samples and facilitates the handling of long-range information while maintaining the base model structure. Spectral Attention preserves long-period trends through a low-pass filter and facilitates gradient to flow between samples. Spectral Attention can be seamlessly integrated into most sequence models, allowing models with fixed-sized look-back windows to capture long-range dependencies over thousands of steps. Through extensive experiments on 11 real-world time series datasets using 7 recent forecasting models, we consistently demonstrate the efficacy of our Spectral Attention mechanism, achieving state-of-the-art results.

==> tables/short_main.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[]
\centering
\caption{Forecasting results for prediction lengths $S \in \{96, 192, 336, 720\}$ with a fixed look-back window $T = \{96\}$. All experiments are conducted with three seeds. The results represent the average across all prediction lengths, except for the Exchange dataset, which includes prediction lengths of $S \in \{96\}$ due to its short data length. Full results are provided in Appendix \ref {appen:result1-1}.}
\vspace{5pt}
\label{tab:short_main}
\resizebox{1.0\textwidth}{!}{%
\begin{tabular}{@{}cc|c|cccccccc|ll@{}}
\toprule
\multicolumn{2}{c|}{Model} & Metric & Weather & Traffic & ECL & ETTh1 & ETTh2 & ETTm1 & ETTm2 & Exchange & Average & p-value \\ \midrule
\multicolumn{1}{c|}{} &  & MSE & 0.2444 & 0.7367 & 0.2266 & 0.5294 & 0.3488 & 0.4617 & 0.2475 & 0.0880 & 0.3886 &  \\
\multicolumn{1}{c|}{} & \multirow{-2}{*}{base} & MAE & 0.3084 & 0.4513 & 0.3245 & 0.5075 & 0.4056 & 0.4470 & 0.3321 & 0.2110 & 0.3789 &  \\ \cmidrule(l){2-13} 
\multicolumn{1}{c|}{} &  & MSE & {\color[HTML]{000000} \textbf{0.2196}} & {\color[HTML]{000000} \textbf{0.6906}} & {\color[HTML]{000000} \textbf{0.2166}} & {\color[HTML]{000000} \textbf{0.5265}} & {\color[HTML]{000000} \textbf{0.3409}} & {\color[HTML]{000000} \textbf{0.4414}} & {\color[HTML]{000000} \textbf{0.2205}} & {\color[HTML]{000000} \textbf{0.0810}} & \textbf{0.3692} & {\color[HTML]{ff0000}\textless{} 0.001} \\
\multicolumn{1}{c|}{\multirow{-4}{*}{DLinear}} & \multirow{-2}{*}{BSA} & MAE & {\color[HTML]{000000} \textbf{0.2815}} & {\color[HTML]{000000} \textbf{0.4354}} & {\color[HTML]{000000} \textbf{0.3164}} & {\color[HTML]{000000} \textbf{0.5070}} & {\color[HTML]{000000} \textbf{0.3977}} & {\color[HTML]{000000} \textbf{0.4469}} & {\color[HTML]{000000} \textbf{0.3104}} & {\color[HTML]{000000} \textbf{0.2070}} & \textbf{0.3692} & 0.658 \\ \midrule
\multicolumn{1}{c|}{} &  & MSE & 0.2480 & 0.7226 & 0.2308 & 0.5512 & 0.3087 & 0.4880 & 0.2204 & 0.0852 & 0.3849 &  \\
\multicolumn{1}{c|}{} & \multirow{-2}{*}{base} & MAE & 0.2736 & 0.4415 & 0.3195 & \textbf{0.5156} & 0.3702 & 0.4570 & 0.3067 & 0.2036 & 0.3773 &  \\ \cmidrule(l){2-13} 
\multicolumn{1}{c|}{} &  & MSE & {\color[HTML]{000000} \textbf{0.2366}} & {\color[HTML]{000000} \textbf{0.6654}} & {\color[HTML]{000000} \textbf{0.2125}} & {\color[HTML]{000000} \textbf{0.5446}} & {\color[HTML]{000000} \textbf{0.3039}} & {\color[HTML]{000000} \textbf{0.4746}} & {\color[HTML]{000000} \textbf{0.2101}} & {\color[HTML]{000000} \textbf{0.0851}} & \textbf{0.3681} & {\color[HTML]{ff0000}\textless{} 0.001} \\
\multicolumn{1}{c|}{\multirow{-4}{*}{RLinear}} & \multirow{-2}{*}{BSA} & MAE & {\color[HTML]{000000} \textbf{0.2667}} & {\color[HTML]{000000} \textbf{0.4043}} & {\color[HTML]{000000} \textbf{0.3009}} & {\color[HTML]{000000} 0.5172} & {\color[HTML]{000000} \textbf{0.3701}} & {\color[HTML]{000000} \textbf{0.4530}} & {\color[HTML]{000000} \textbf{0.3026}} & {\color[HTML]{000000} \textbf{0.2035}} & \textbf{0.3677} & {\color[HTML]{ff0000}\textless{} 0.001} \\ \midrule
\multicolumn{1}{c|}{} &  & MSE & 0.2399 & 0.5267 & 0.1952 & 0.5128 & 0.3098 & 0.4597 & \textbf{0.2337} & 0.0953 & 0.3451 &  \\
\multicolumn{1}{c|}{} & \multirow{-2}{*}{base} & MAE & \textbf{0.2858} & 0.3224 & \textbf{0.2846} & 0.5063 & 0.3925 & 0.4503 & \textbf{0.3213} & 0.2318 & 0.3616 &  \\ \cmidrule(l){2-13} 
\multicolumn{1}{c|}{} &  & MSE & {\color[HTML]{000000} \textbf{0.2355}} & {\color[HTML]{000000} \textbf{0.5020}} & {\color[HTML]{000000} \textbf{0.1923}} & {\color[HTML]{000000} \textbf{0.5107}} & {\color[HTML]{000000} \textbf{0.3075}} & {\color[HTML]{000000} \textbf{0.4305}} & {\color[HTML]{000000} 0.2407} & {\color[HTML]{000000} \textbf{0.0893}} & \textbf{0.3368} & {\color[HTML]{ff0000}0.004} \\
\multicolumn{1}{c|}{\multirow{-4}{*}{FreTS}} & \multirow{-2}{*}{BSA} & MAE & {\color[HTML]{000000} 0.2923} & {\color[HTML]{000000} \textbf{0.3167}} & {\color[HTML]{000000} 0.2866} & {\color[HTML]{000000} \textbf{0.5053}} & {\color[HTML]{000000} \textbf{0.3875}} & {\color[HTML]{000000} \textbf{0.4422}} & {\color[HTML]{000000} 0.3259} & {\color[HTML]{000000} \textbf{0.2193}} & \textbf{0.3602} & 0.392 \\ \midrule
\multicolumn{1}{c|}{} &  & MSE & 0.2596 & \textbf{0.6199} & 0.2028 & 0.5757 & 0.3856 & 0.5077 & 0.2469 & 0.0943 & 0.3808 &  \\
\multicolumn{1}{c|}{} & \multirow{-2}{*}{base} & MAE & 0.2840 & \textbf{0.3331} & 0.3011 & 0.5453 & 0.4266 & 0.4819 & 0.3257 & 0.2187 & 0.4034 &  \\ \cmidrule(l){2-13} 
\multicolumn{1}{c|}{} &  & MSE & {\color[HTML]{000000} \textbf{0.2516}} & 0.6237 & \textbf{0.1985} & {\color[HTML]{000000} \textbf{0.5693}} & {\color[HTML]{000000} \textbf{0.3783}} & {\color[HTML]{000000} \textbf{0.4991}} & {\color[HTML]{000000} \textbf{0.2295}} & {\color[HTML]{000000} \textbf{0.0941}} & \textbf{0.3717} & {\color[HTML]{ff0000}0.017} \\
\multicolumn{1}{c|}{\multirow{-4}{*}{TimesNet}} & \multirow{-2}{*}{BSA} & MAE & {\color[HTML]{000000} \textbf{0.2792}} & 0.3348 & \textbf{0.2976} & {\color[HTML]{000000} \textbf{0.5404}} & {\color[HTML]{000000} \textbf{0.4176}} & {\color[HTML]{000000} \textbf{0.4764}} & {\color[HTML]{000000} \textbf{0.3139}} & {\color[HTML]{000000} \textbf{0.2186}} & \textbf{0.3966} & {\color[HTML]{ff0000}0.005} \\ \midrule
\multicolumn{1}{c|}{} &  & MSE & 0.2556 & \textbf{0.4276} & 0.1811 & 0.5416 & 0.3206 & 0.4664 & 0.2238 & 0.0905 & 0.3365 &  \\
\multicolumn{1}{c|}{} & \multirow{-2}{*}{base} & MAE & 0.2766 & \textbf{0.2843} & 0.2723 & 0.5175 & 0.3797 & 0.4538 & 0.3145 & 0.2115 & 0.3519 &  \\ \cmidrule(l){2-13} 
\multicolumn{1}{c|}{} &  & MSE & {\color[HTML]{000000} \textbf{0.2357}} & {\color[HTML]{000000} 0.4283} & {\color[HTML]{000000} \textbf{0.1760}} & {\color[HTML]{000000} \textbf{0.5367}} & {\color[HTML]{000000} \textbf{0.3166}} & {\color[HTML]{000000} \textbf{0.4663}} & {\color[HTML]{000000} \textbf{0.2189}} & {\color[HTML]{000000} \textbf{0.0898}} & \textbf{0.3311} & {\color[HTML]{ff0000}0.001} \\
\multicolumn{1}{c|}{\multirow{-4}{*}{iTransformer}} & \multirow{-2}{*}{BSA} & MAE & {\color[HTML]{000000} \textbf{0.2682}} & {\color[HTML]{000000} 0.2885} & {\color[HTML]{000000} \textbf{0.2697}} & {\color[HTML]{000000} \textbf{0.5171}} & {\color[HTML]{000000} \textbf{0.3784}} & {\color[HTML]{000000} \textbf{0.4524}} & {\color[HTML]{000000} \textbf{0.3099}} & {\color[HTML]{000000} \textbf{0.2106}} & \textbf{0.3499} & {\color[HTML]{ff0000}0.015} \\ \midrule
\multicolumn{1}{c|}{} &  & MSE & 0.2400 & 0.5377 & \textbf{0.1501} & \textbf{0.5174} & 0.3234 & 0.4849 & \textbf{0.2426} & 0.2199 & 0.3532 &  \\
\multicolumn{1}{c|}{} & \multirow{-2}{*}{base} & MAE & 0.2921 & 0.2793 & \textbf{0.2467} & \textbf{0.5199} & 0.4024 & 0.4698 & 0.3424 & 0.3451 & 0.3801 &  \\ \cmidrule(l){2-13} 
\multicolumn{1}{c|}{} &  & MSE & {\color[HTML]{000000} \textbf{0.2267}} & {\color[HTML]{000000} \textbf{0.5342}} & {\color[HTML]{000000} 0.1524} & {\color[HTML]{000000} 0.5203} & {\color[HTML]{000000} \textbf{0.3167}} & {\color[HTML]{000000} \textbf{0.4678}} & {\color[HTML]{000000} 0.2452} & {\color[HTML]{000000} \textbf{0.2188}} & \textbf{0.3480} & {\color[HTML]{ff0000}0.039} \\
\multicolumn{1}{c|}{\multirow{-4}{*}{Crossformer}} & \multirow{-2}{*}{BSA} & MAE & {\color[HTML]{000000} \textbf{0.2837}} & {\color[HTML]{000000} \textbf{0.2775}} & {\color[HTML]{000000} 0.2503} & {\color[HTML]{000000} 0.5216} & {\color[HTML]{000000} \textbf{0.3962}} & {\color[HTML]{000000} \textbf{0.4692}} & {\color[HTML]{000000} \textbf{0.3399}} & {\color[HTML]{000000} \textbf{0.3399}} & \textbf{0.3775} & {\color[HTML]{ff0000}0.042} \\ \midrule
\multicolumn{1}{c|}{} &  & MSE & 0.2553 & \textbf{0.4672} & 0.1983 & \textbf{0.5352} & 0.3172 & 0.4731 & 0.2204 & 0.0867 & 0.3432 &  \\
\multicolumn{1}{c|}{} & \multirow{-2}{*}{base} & MAE & 0.2776 & \textbf{0.2962} & 0.2861 & \textbf{0.5161} & 0.3745 & 0.4562 & 0.3101 & 0.2035 & 0.3542 &  \\ \cmidrule(l){2-13} 
\multicolumn{1}{c|}{} &  & MSE & {\color[HTML]{000000} \textbf{0.2356}} & {\color[HTML]{000000} 0.4672} & {\color[HTML]{000000} \textbf{0.1894}} & {\color[HTML]{000000} 0.5388} & {\color[HTML]{000000} \textbf{0.3143}} & {\color[HTML]{000000} \textbf{0.4575}} & {\color[HTML]{000000} \textbf{0.2142}} & {\color[HTML]{000000} \textbf{0.0856}} & \textbf{0.3363} & {\color[HTML]{ff0000}\textless{} 0.001} \\
\multicolumn{1}{c|}{\multirow{-4}{*}{PatchTST}} & \multirow{-2}{*}{BSA} & MAE & {\color[HTML]{000000} \textbf{0.2683}} & {\color[HTML]{000000} 0.2969} & {\color[HTML]{000000} \textbf{0.2850}} & {\color[HTML]{000000} 0.5198} & {\color[HTML]{000000} \textbf{0.3744}} & {\color[HTML]{000000} \textbf{0.4508}} & {\color[HTML]{000000} \textbf{0.3058}} & {\color[HTML]{000000} \textbf{0.2023}} & \textbf{0.3519} & {\color[HTML]{ff0000}0.015} \\ \bottomrule
\end{tabular}%
}
\vspace{-10pt}
\end{table}
